Linearly Mapping from Image to Text Space

The extent to which text-only language models (LMs) learn to represent features of the non-linguistic world is an open question. Prior work has shown that pretrained LMs can be taught to caption images when a vision model's parameters are optimized to encode images in the language space. We test a stronger hypothesis: that the conceptual representations learned by frozen text-only models and vision-only models are similar enough that this can be achieved with a linear map. We show that the image representations from vision models can be transferred as continuous prompts to frozen LMs by training only a single linear projection. Using these to prompt the LM achieves competitive performance on captioning and visual question answering tasks compared to models that tune both the image encoder and text decoder (such as the MAGMA model). We compare three image encoders with increasing amounts of linguistic supervision seen during pretraining: BEIT (no linguistic information), NF-ResNET (lexical category information), and CLIP (full natural language descriptions). We find that all three encoders perform equally well at transferring visual property information to the language model (e.g., whether an animal is large or small), but that image encoders pretrained with linguistic supervision more saliently encode category information (e.g., distinguishing hippo vs. elephant) and thus perform significantly better on benchmark language-and-vision tasks. Our results indicate that LMs encode conceptual information structurally similarly to vision-based models, even those that are solely trained on images. Code is available here: https://github.com/jmerullo/limber

==> sections/results.tex <==
\section{Results}
We evaluate our models' abilities to generate relevant or related content of an image with automatic captioning and visual question answering benchmarks. Both tasks are framed as open-ended generative tasks that rely on the LM's ability to map image prompts to a coherent and realistic sentences describing that image. First, we establish that freezing $E$ and $L$ and tuning $P$ produces coherent and relevant captions comparable to Frozen and MAGMA and other fully tuned image captioning models. Following that, we specifically look for differences between the captions generated by models with different choices of $E$ and performance on downstream reasoning with visual question answering. We hypothesize that the more linguistic supervision a model has, the better its overall transferability to the LM will be, and thus the better captions or generated answers to questions will be. However, it could be the case that that specific concepts transfer more easily from a vision-only model, so we additionally analyze fine-grained conceptual information within a corpus of generated captions.
\subsection{Image Captioning}
\label{sec:captioning}
\begin{table}[h!]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|cccc|clcl|c|cc|}
\hline
Model & \multicolumn{4}{c|}{NoCaps - CIDEr-D} & \multicolumn{4}{c|}{NoCaps (All)} & CoCo & \multicolumn{2}{c|}{CoCo} \\
 & In & Out & Near & All & \multicolumn{2}{c}{CLIP-S} & \multicolumn{2}{c|}{Ref-S} & CIDEr-D & CLIP-S & Ref-S \\ \hline
\emoji{fire} NFRN50$_{tuned}$ & 20.9 & 30.8 & 25.3 & 27.3 & \multicolumn{2}{c}{66.5} & \multicolumn{2}{c|}{72.5} & 35.3 & \multicolumn{1}{c|}{69.7} & 74.8 \\
\emoji{fire} MAGMA (released) & 18.0 & 12.7 & 18.4 & 16.9 & \multicolumn{2}{c}{63.2} & \multicolumn{2}{c|}{68.8} & \textbf{52.1} & \multicolumn{1}{c|}{\textbf{76.7}} & 79.4 \\
\emoji{fire} MAGMA (ours) & \textbf{30.4} & \textbf{43.4} & \textbf{36.7} & \textbf{38.7} & \multicolumn{2}{c}{\textbf{74.3}} & \multicolumn{2}{c|}{\textbf{78.7}} & 47.5 & \multicolumn{1}{c|}{75.3} & \textbf{79.6} \\ \hline
\emoji{snowflake}NFRN50$_{random}$ & 5.4 & 4.0 & 4.9 & 5.0 & \multicolumn{2}{c}{47.5} & \multicolumn{2}{c|}{55.7} & 4.8 & \multicolumn{1}{c|}{49.5} & 57.1 \\
\emoji{snowflake}BEIT & 20.3 & 16.3 & 18.9 & 18.9 & \multicolumn{2}{c}{62.0} & \multicolumn{2}{c|}{69.1} & 22.3 & \multicolumn{1}{c|}{63.6} & 70.0 \\
\emoji{snowflake}NFRN50 & 21.3 & 31.2 & 26.9 & 28.5 & \multicolumn{2}{c}{65.6} & \multicolumn{2}{c|}{71.8} & 36.2 & \multicolumn{1}{c|}{68.9} & 74.1 \\
\emoji{snowflake}CLIP & \textbf{34.3} & \textbf{48.4} & \textbf{41.6} & \textbf{43.9} & \multicolumn{2}{c}{\textbf{74.7}} & \multicolumn{2}{c|}{\textbf{79.4}} & \textbf{54.9} & \multicolumn{1}{c|}{\textbf{76.2}} & \textbf{80.4} \\ \hline
\end{tabular}
}%
\caption{Captioning performance for all variations on model architecture and image encoder used. Ref-S refers to RefCLIP Score.}
\label{tab:caption_results}
\end{table}

We evaluate the ability of each model to generate an accurate description of an image. We test on the CoCo \citep{coco} and NoCaps \citep{nocaps} datasets. Following convention from \textit{SimVLM} and MAGMA, we input the prefix "A picture of" after every image to prompt the model. Like in previous work, we find that this is a favorable prompt which tends to increase performance. 
We evaluate multiple captioning metrics. We report CIDEr-D (more commonly referred to as just CIDEr) \citep{cider}, CLIPScore, and RefCLIPScore \citep{hessel2021clipscore} metrics in Table \ref{tab:caption_results}. Full captioning results including other metrics can be found in Appendix \ref{sec:caption_appendix}. In contrast to previous work \citep{vladapter}, only training $P$ and not tuning the parameters of $LM$ does not seem to hurt caption generation and in some cases helps when comparing frozen CLIP vs. full MAGMA training. We find that CLIPScore is a preferable metric for our use case since it does not compare the generation to a ground truth caption, rather it computes the cosine similarity between CLIP's encoding of the image and produced caption, which we hypothesize will reward higher semantic similarity between the text and the image, even if the generated text does not compare favorably to the ground truth caption in terms of token overlap.

Intuitively, we find that models trained to transfer multimodal CLIP encodings perform the best, while the model trained with the BEIT encoder, which has no linguistic supervision, performs the worst of the pretrained image encoders. However, BEIT performs notably better than the randomly initialized NFResnet50, indicating that the concepts learned in vision pretraining are transferring to the language model, instead of just learning a naive mapping between visual trends during prompt tuning. This result offers some evidence in favor of the hypothesis that language model representations are \textit{isomorphic} to those of a grounded world, but it appears to be limited. We further investigate which concepts specifically transfer better than others in the following sections.

\subsection{Visual Question Answering}
\label{sec:vqa}
\begin{table}[ht]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|}
\hline
Model & 0 & 1 & 2 & 4 \\ \hline
Blind & 20.60 & 35.11 & 36.17 & 36.99 \\ \hline
NFResnet50 tuned & 27.15 & 37.47 & 38.48 & 39.18 \\
MAGMA (ours) & 24.62 & 39.27 & 40.58 & 41.51 \\
MAGMA (reported) & \textbf{32.7} & \textbf{40.2} & \textbf{42.5} & \textbf{43.8} \\ \hline
NFResnet50 random & 25.34 & 36.15 & 36.79 & 37.43 \\
BEIT & 24.92 & 34.35 & 34.70 & 31.72 \\
NFResnet50 & 27.63 & 37.51 & 38.58 & 39.17 \\
CLIP & \textbf{33.33} & \textbf{39.93} & \textbf{40.82} & \textbf{40.34} \\ \hline
MAGMA (released) & 33.48 & 43.19 & 44.85 & 45.65 \\ \hline
\end{tabular}
}
\caption{Few-shot performance on VQA dataset for each model. We differentiate the released and reported MAGMA models from \citet{magma} because the authors report a variant of the MAGMA model on VQA 2.0 which is the more comparable to the one we train than the one available on Huggingface.}
\label{tab:vqa_table}
\end{table}
\citet{frozen, magma, vladapter} all show strong few-shot performance with in-context examples answering questions about image properties. We perform similar experiments to test how well different image encoders transfer specific details or visual properties necessary to answer the questions. We use the VQA 2.0 dataset \citep{balanced_vqa_v2} which, in the validation split, contains over 200k questions for 40.5k images and allows us to test for understanding of a wide range of concepts. Visual question answering can also help us gauge which fine-grained concepts are collapsed or unable to transfer to the language model with only a linear transformation. We follow the few-shot procedure used in \citet{magma} in which we prompt the models with the ``[image] Q: [q] A:" format. We take the first word of the generation and, like in the MAGMA paper, truncate to the length of the longest ground truth answer. We also use the normalization procedure described in the VQA repo\footnote{https://github.com/GT-Vision-Lab/VQA}. Our results can be seen in Table \ref{tab:vqa_table}. Like with the captioning results, we find that scores gradually increase as the linguistic supervision the image encoder saw in pretraining gets richer. Interestingly, we find that the BEIT model can not outperform the Blind or random ResNet baselines: in the 4-shot setting, BEIT underperforms by around 6\%. This is surprising considering that based on our captioning evaluation, BEIT prompts generate much stronger captions than those produced by the random ResNet. While the blind model can only make guesses based off of the inferred label distribution of the text, random ResNet and BEIT are both given images. We consider this telling that while the LM can recover basic concepts from the BEIT encodings, if BEIT \textit{does} encode a hierarchy or taxonomy of visual concepts for the details of a given image, it can not be transferred linearly. Since BEIT is our only exclusively visual model, this suggests that finer-grained details, such as those required to reason over an image to answer basic questions or animal \textit{type} as discussed in the previous section, are not represented isomorphically to language model representations, adding nuance to the idea that language models can learn conceptually grounded embeddings without actually being grounded.

[TODO: bootstraps, more random seeds]

%As our results show, training a projection from a frozen CLIP outperforms our MAGMA implementation on average, especially in the zero-shot case. Looking at the breakdown of question types (See Appendix \ref{tab:all_vqa_qtypes}), we find that CLIP does better on almost all question types, but not by a dramatic amount on any categories. 

NOTES: -----\\

Finetuning $E$ and $LM$ (as is done in MAGMA training) has a significant impact on ``how many people are in..." type questions
%an over 10 percent increase on average for three types of questions: \{\textit{``are these", ``is there", ``how many people are in"} \} type questions. 
%These question types all revolve around identifying and connecting content in the image to the outside world (``Are these art pieces handmade?"), identifying details within the image (``Is there frost on the ground?"), and counting (``How many people are in this picture?") respectively.
Despite overall better performance, there are no question types in which CLIP outperforms our version MAGMA by such a wide margin. On the other hand, tuning Resnet does not increase performance on any question types over freezing Resnet by a large amount\footnote{Tuning Resnet grants a 4 point increase on "What room is" questions, which ask to identify whether a room is a kitchen, living room, etc. and is statistically significant (p<.01) on a Wilcoxon signed-rank test.}, suggesting that the increase in performance from Frozen CLIP to MAGMA is due to the parameters tuned in the language model adapters. Further analysis is needed to confirm whether this applies to any image encoder used, but do to computational constraints we could not carry out all model component ablations. 

CLIP based models are much better at questions like ``What are they baking?" or ``What is the person doing with the laptop?". Can connect the image to the action/has a word for it? For the latter, the Frozen CLIP is over 20 points higher than the next highest non-clip model (NFRN50). Similar story with "what is in the" questions.

All of the tested models are bad at answering ``why" questions like ``Why does the bus have to stop?" suggesting either an inability to infer about the world in this way or because of the difficulty of generating an answer that matches the ground truth exactly.

Pretrained ResNet models are statistically significantly ($p<.01$) better at answering ``how many" of an object are present in an image than the other models we trained, including the CLIP based models. The gap closes slightly by tuning CLIP and adapters in our MAGMA implementation, so is the information still present in the projection, and just requires additionaly training to teach the model how to extract it?

\begin{table*}[ht]
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Model & SPICE (All) & Relations & Cardinality & Attributes & Size & Color & Object \\ \hline
NFResnet50 tuned & 9.1 & 1.12 & 0.02 & 1.64 & 0.33 & 0.40 & 19.9 \\
MAGMA (ours) & 11.0 & 1.37 & 0.00 & 3.94 & 0.36 & 1.31 & 22.6 \\
MAGMA (released) & \textbf{11.7} & \textbf{1.99} & \textbf{1.30} & \textbf{3.95} & \textbf{0.50} & \textbf{1.32} & \textbf{23.8} \\ \hline
NFResnet50 random & 2.14 & 0.06 & 0.00 & 0.22 & 0.00 & 0.12 & 4.93 \\
BEIT & 6.4 & 0.61 & 0.0 & 1.26 & 0.21 & 0.45 & 14.1 \\
NFResnet50 & 9.28 & 1.28 & 0.02 & 1.70 & 0.27 & 0.42 & 20.2 \\
CLIP & \textbf{12.1} & \textbf{1.83} & \textbf{0.08} & \textbf{3.76} & \textbf{0.39} & \textbf{0.75} & \textbf{25.08} \\ \hline
\end{tabular}
}%
\caption{F-scores (x100) for each fine-grained category of the SPICE metric, evaluated on the 2017 COCO validation dataset. The top and bottom divide separates models where the image encoder is either tuned of frozen, respectively. Models that use CLIP as their image encoder show a large jump in improvement over other models (even compared to tuned ResNet), especially in the Attributes (e.g. adjectives) and Object (e.g. nouns) categories.}
\label{tab:spice_results}
\end{table*}

\subsection{Fine-grained Analysis of Concept Transfer}
\label{sec:fine_grained_captions}
The SPICE metric \citep{anderson2016spice} works by creating a scene graph from ground truth and candidate captions and compares their similarities. This allows us to get scores for how well each of our models' captions generate fine-grained features like nouns (objects), the relations between them (e.g. verbs), and the modifiers (e.g. adjectives) describing them. It has also been shown that SPICE correlates more strongly with captions that are absent of hallucinations than other image-captioning metrics \citep{rohrbach2018object}. The results can be seen in Table \ref{tab:spice_results}. We find that models trained with frozen image encoders perform similarly well to those with additional parameters tuned, but models that do better on other metrics tend to do better at recovering scene graphs in SPICE. We don't find convincing reason to believe that prompt tuning provides a strong enough signal to update the representations of the vision model in a useful way when compared to just freezing it. We find that all of the models do a good job of recovering the objects in an image, but there is a steep drop going from Resnet to BEIT, suggesting that the linguistic supervision in Resnet and CLIP pretraining helps distinguish objects into class categories that can more easily be transferred to an LM. Since object classification provides an object label corresponding to a word this makes sense, however \citet{bao2021beit} show that BEIT's pretraining specifically enables it to transfer to image classification and semantic segmentation very well, so the interpretation is that it is not linearly transferable to the LM [NOTE: or it is not linearly recoverable from the model, a probing experiment could eliminate that].  We see even steeper drop offs with relations and attributes going from CLIP to the other models, which follows from the fact that CLIP learns to align descriptions of objects and actions in images to text. The question remains however, as to whether specific concepts within one category transfer more easily than others, and if such concepts differs between different models. Given that Resnet and BEIT weights used were both pretrained on ImageNet-1k, the only differences should be due to architecture and pretraining task.



\begin{figure}
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{iclr2023/figures/captions/recall_wup_obj_category.pdf}
         \caption{Recall for each model across object categories in generated captions. The improvement over the recall given as the Wu-Palmer Similarity is shown as the gray stacked bars. Although BEIT is worse at generating the exact right word for each caption, the semantic similarity of generated objects brings it up to the performance of more linguistically informed models in several categories.}
         \label{fig:recall_wup_stacked}
     \end{subfigure}
\end{figure}
     

In order to understand where transfer succeeds and fails, we examine the likelihood that a given model will generate a specific concept conditioned on the fact that it shows up in a ground truth caption for some image. We look at the most common objects, modifiers (e.g. adjectives), and relations (e.g. verbs) in the ground truth captions and how often each model predicts them. We take the 50 most common object/modifier/relation words that appear in the ground truth captions, and organize them by category. We then look at the rate at which each model with a frozen image encoder generates a caption that contains that word using the F1 score. Notably, examining the data this way reveals that BEIT struggles in ways unique from the other models. While CLIP and Resnet based models have very high performance for recognizing specific animals in an image, BEIT fails to do so reliably, exhibiting a starker deficit here than in the other categories of objects. The Wu-Palmer Similarity (WuP) [cite] can be used to measure the similarity of two words in $[0,1]$ using their location in the WordNet hierarchy, based on the location of the most-specific-ancestor of two words. The WuP score, in this instance, can be considered a `soft' recall, because it offers a way for a model to score highly, even if it didn't predict the exact correct word. For example, predicting `cat' when given a picture of a tiger is correct in the sense that it predicted a noun under the same general family, and would receive a higher WuP score than predicting `chair'. We compare the recall and WuP score on average for each category, and report them in Figure \ref{fig:recall_wup_stacked}. Detailed analyses including F1 and scores for each individual word we tested, including on the tuned image encoder models can be found in Appendix \ref{sec:caption_appendix}. We find that, on average, BEIT scores much lower in terms of recall, but makes up much of the ground in terms of semantic similarity when measured with WuP. BEIT closes the distance, and sometimes outperforms the more linguistically informed models in terms of average similarity. This supports the idea that BEIT is able to transfer broad semantic content, but can not specify to the language model specific word forms that the other models explicitly learned (either directly or indirectly) during vision pretraining. In Section \ref{sec:probe_img} we show that this information is not present in BEIT representations to begin with, and is not a failure of the language model to linearly transfer this information.

\section{Controlling for Vision Representation Quality}
\label{sec:probe_img}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{iclr2023/figures/probes/probe_f1_by_mean_supercategory.pdf}
    \caption{F1 for each probe trained on representations from the corresponding image encoders. Note that each probe is trained to classify each of the 80 object categories in COCO but here we aggregate over each provided `supercategory' for visualization.}
    \label{fig:f1_probes}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{iclr2023/figures/probes/beit_animal_f1.pdf}
    \caption{BEIT Animal}
    \label{fig:beit_animal_probe_caption}
\end{figure}

\citet{desai2021virtex} argue that captions are a strong signal for learning visual representations because they are more \textit{semantically dense} than image classification labels. By extension, image classification labels are more semantically dense than no supervision at all. An alternative explanation for the general `vagueness' of the generated captions from a vision-only model like BEIT, is that its representations support less semantic density (particularly that which can be aligned with language) in the first place. 

To investigate this, we perform a linear probing task on the frozen image encoder representations to probe for the existence of conceptual information present in an image. Previously, we showed that some concepts do not linearly \textit{transfer} to the LM from the vision space. In short, this experiment tests to see if such concepts are \textit{encoded} linearly in the vision representations at all. If the fine-grained detail can not be learned by a linear probe, then we can not expect that such detail would be linearly transferable to the LM input space. For this task, we train probes on the image representations before they are projected into the language model; one for each image encoder. Each probe is trained on the training set of the COCO image captioning dataset ($\sim$100k images) and evaluated on the validation set ($\sim$5k images) on a multilabel object classification task. The object labels are derived from the object segmentation labels for each image.

\paragraph{Linearly Encoded vs. Linearly Transferable} The results from our probing experiments can be found in Figure \ref{fig:f1_probes}. We use this experiment to draw the distinction between a concept being \textit{linearly encoded} vs. being \textit{linearly transferable}. The former implies that a concept is encoded in the image representations and a linear probe can learn to classify images as either containing that concept or not. ``Linearly transferable", on the other hand, refers to how successfully the language model can take an image prompt projected into its input space, recognize the concepts in the prompt, and generate an appropriate caption. Overall, we find that the ability of the probe is proportional to the performance of the downstream captions, suggesting that if the the concept is linearly encoded, then it is likely to be transferable to the language model. This is important because it suggests that the lacking performance BEIT prompts have on captioning and VQA tasks may not be due to  poor transferability, but that BEIT representations do not consistently encode these concepts.  

We do find some evidence of concepts which are linearly encoded, but not transferable. For example, in Figure \ref{fig:beit_animal_probe_caption}, we highlight the F1 score of BEIT for the probe classification task as well as the F1 of the model generating the object class in a caption for the \textbf{animals} category. We pick animals specifically because it is completely unambiguous how the model should refer to them in captions (e.g. as opposed to `man', `woman', `boy', `girl' for people) and because of the previous finding that BEIT tends to struggle with specific types of animals compared to other models. The gap between `giraffe' for example with BEIT representations seems to imply that the concept is linearly encoded, but not transferable to the language model. Since CLIP and NFRN50 have very high performance on captioning giraffes (0.975 and 0.866 F1 respectively), we know this is not due to a lack of exposure to the giraffe concept in training the image projection\footnote{BEIT and NFRN50 were both pretrained on ImageNet, so it is not due to a lack of exposure in vision pretraining either}.

[TODO: move this to the appendix] collect image representations for the CIFAR-100 dataset \citep{cifar100} for the random NFRN50, pretrained NFRN50, BEIT, and CLIP image encoders. This dataset contains 60k training images of objects that are labeled for one of 100 fine-grained object classes and one of 20 coarse grained classes, which we can use as labels in a linear probing task performed on the image representations. We use 100 images from each fine class from the training set as a validation set (40k train, 10k validation). We use the balanced 10k image test set provided by the authors to report our results.
%*NFRN better at "who is"
%*CLIP based models better at reading like "what number is"
%* BEIT sucks at 'which'
%* CLIP based much better at "what are"/"What is the person"
%* Everything is bad at "where is the"
%* BEIT better than rand at "what sport is"


%NOTE: given prompt waywardness, it is impossible to evaluate single continuous prompts in the input space of the language model, however, since we can track the movement from visual space to where they end up in language space, the relationship between prompts may be meaningful.

%https://arxiv.org/pdf/2112.03204.pdf show that even prompt tuning for text tasks is unable to fully memorize a dataset



